$f$-GAIL: Learning $f$-Divergence for Generative Adversarial Imitation Learning

Imitation learning (IL) aims to learn a policy from expert demonstrations that minimizes the discrepancy between the learner and expert behaviors. Various imitation learning algorithms have been proposed with different pre-determined divergences to quantify the discrepancy. This naturally gives rise to the following question: Given a set of expert demonstrations, which divergence can recover the expert policy more accurately with higher data efficiency? In this work, we propose $f$-GAIL, a new generative adversarial imitation learning (GAIL) model, that automatically learns a discrepancy measure from the $f$-divergence family as well as a policy capable of producing expert-like behaviors. Compared with IL baselines with various predefined divergence measures, $f$-GAIL learns better policies with higher data efficiency in six physics-based control tasks.

==> background.tex <==
\textbf{Preliminaries  }
In a Markov decision process (MDP) represented as a 6-tuple $\langle {\cal S}, {\cal A}, {\cal P}, c, \rho_0, \gamma \rangle$ where $\mathcal{S}$ is a set of states, $\mathcal{A}$ is a set of actions, ${\cal P}: \mathcal{S}\times\mathcal{A}\times\mathcal{S}\mapsto [0,1]$ is the transition probability distribution, $c:\mathcal{S}\times\mathcal{A}\mapsto\mathbb{R}$ is the cost function, $\rho_0:\mathcal{S}\mapsto\mathbb{R}$ is the distribution of the initial state $s_0$, and $\gamma \in [0, 1]$ is the discount factor informing importance difference between future and present costs. 
In IL, the cost function $c$ is unknown. In this work, we denote the expert policy as $\pi_E$, the learner policy as $\pi$, the set of policies is $\Pi$, and the occupancy measure (i.e. the marginal state-action distribution) of a policy $\pi$ by $\rho^\pi(s,a)$\footnote{The marginal distributions of a policy are obtained by generating infinitely many trajectories with a given policy and computing the frequency of $(s,a)$.}. 
In addition, we use an expectation with respect to a policy $\pi$ to denote an expectation with respect to the trajectories $\pi$ generates: $\mathbb{E}_\pi[g(s,a)]\triangleq \mathbb{E}[\sum_{t=0}^\infty\gamma^t g(s_t,a_t)]$, where $s_0\sim\rho_0,a_t\sim\pi(a_t|s_t),s_{t+1}\sim\mathcal{P}(s_{t+1}|s_t,a_t)$ and here $g$ represents any function.

\textbf{Generative adversarial imitation learning  } Generative adversarial imitation learning (GAIL) \cite{GAIL} solves the IL problem and chooses policies with maximized causal entropy $\mathcal{H}(\pi) = \mathbb{E}_{\pi}[\log\pi(a|s)]$. Let $\mathcal{C}$ be the set of cost functions, % and $\rho^{\pi}$ and $\rho^{\pi_E}$ be the occupancy measures of learner policy $\pi$ and expert policy $\pi_E$ respectively, 
IL approaches begin with the following inverse reinforcement learning (IRL) objective:
\begin{equation*}
   \mathrm{IRL}_\psi(\pi_E)  = \arg \max_{c\in\mathcal{C}} -\psi(c) 
   + \big( \min_{\pi\in\Pi} -\mathcal{H}(\pi) + \mathbb{E}_{\pi}[c(s,a)]\big)-
         \mathbb{E}_{{\pi_E}}[c(s,a)],
\end{equation*}{}
where $\psi:\mathcal{R}\mapsto\mathbb{R}$ is a convex regularization function on the space of cost functions. Given the optimal cost function returned by $\mathrm{IRL}_\psi(\pi_E)$, IL approaches then do reinforcement learning $\mathrm{RL}(c) = \arg\min_{\pi\in \Pi}-\mathcal{H}(\pi) + \mathbb{E}_{\pi}[c(s,a)]$ to obtain an optimal policy. Instead of doing IRL inside the loops of RL, GAIL \cite{GAIL} shows that
\begin{equation}\label{eq:il}
    \mathrm{RL}\circ\mathrm{IRL}_\psi(\pi_E)  = \arg \min_{\pi\in\Pi} -\mathcal{H}(\pi) + \psi^* (\rho^{\pi}-
         \rho^{\pi_E}),
\end{equation}{}
where $\psi^*$ is the convex conjugate of $\psi$. This implies that the process of inferring expert policy bypassing IRL is equivalent as finding the policy that minimizes the occupancy measure discrepancies measured by $\psi^*$.

With a proper choice of $\psi$ as $\psi_{GA}$\footnote{We refer the readers to Section 5 in GAIL\cite{GAIL} for detailed information of $\psi$ choice.}, the learner policy in GAIL tries to minimize the occupancy measure Jensen-Shannon divergence $D_{JS} (\rho^{\pi}, \rho^{\pi_E}) = \max_{D\in(0, 1)^{\mathcal{S}\times\mathcal{A}}} \mathbb{E}_\pi[\log(D(s,a))] + \mathbb{E}_{{\pi_E}}[\log(1-D(s,a))]$ to the expert policy, i.e.,
\begin{align}\label{eq:GAIL}
    \min_{\pi\in\Pi} & \max_{D\in(0, 1)^{\mathcal{S}\times\mathcal{A}}} \mathbb{E}_\pi[\log(D(s,a))] + \mathbb{E}_{{\pi_E}}[\log(1-D(s,a))]-\mathcal{H}(\pi),
\end{align}{}
%This choice of $\psi$ enables the introduction of adversarial training idea \cite{goodfellow2014generative}: 
where, $D:\mathcal{S}\times\mathcal{A}\mapsto (0,1)$ is a discriminator with final sigmoid activation that distinguishes state-action pairs from expert demonstrations and those generated by the learner policy $\pi$; the learner policy is a generator network that strives to generate expert-like state-action pairs.


\textbf{The $f$-divergence family  }
$f$-Divergence \cite{lin1991divergence,liese2006divergences,csiszar2004information} is a broad family of divergences which measures  discrepancy between two probability distributions, such as  Kullback-Leibler (KL) divergence \cite{kullback1951information}. Given two distributions $P$ and $Q$ with density functions $p(x)$ and $q(x)$ over a finite set of random variables $x\in\mathcal{X}$, where $p(x)$ is absolutely continuous with respect to $q(x)$, the $f$-divergence is defined as
$
    D_f(P||Q) = \sum_{x\in{\cal X}} q(x)f(\frac{p(x)}{q(x)}),
$
where $f: \mathbb{R}^+\mapsto \mathbb{R}$ is a convex. lower semi-continuous function with $f(1)=0$. Different choices of $f$ recover different divergences, e.g. the KL divergence, Jensen-Shannon divergence or total variation divergence. 

Every $f$ in the $f$-divergence family has its \textit{convex conjugate} function $f^*$, also known as \textit{Fenchel conjugate} \cite{hiriart2012fundamentals}: $f^*(t) = \sup_{u\in\mathrm{dom}_f}\{ut-f(u)\}$. With this, we can derive the variational lower bound of a $f$-divergence as $D_f(P||Q)\geq \sup_{t\in\mathrm{dom}_f}\big(\mathbb{E}_{x\sim P}[t] - \mathbb{E}_{x\sim Q}[f^*(t)]\big)$ \cite{nowozin2016f}.

% \textbf{The f-divergence family and variational estimation  }
% $f$-Divergence \cite{lin1991divergence,liese2006divergences,csiszar2004information} measures the difference between two given probability distributions. Given two distributions $P$ and $Q$ with density functions $p(x)$ and $q(x)$ over a finite set of random variables $x\in\mathcal{X}$ where $p(x)$ is absolutely continuous w.r.t. $q(x)$, the $f$-divergence is defined as
% $D_f(P||Q) = \sum_{x\in{\cal X}} q(x)f(\frac{p(x)}{q(x)})$,
% where $f: \mathbb{R}^+\mapsto \mathbb{R}$ is a convex. lower semi-continuous function where $f(1)=0$. Different choices of $f$ recover different divergences, e.g. KL, Jensen-Shannon or Total Variation.

% In \cite{nguyen2010estimating}, the convex conjugate of $f$ function $f^*$ enables a lower bound estimation of the $f$-divergence, 
% \begin{equation}
    
% \end{equation}{}


% \textbf{$f$-GAN  }
\zzrev{Using this variational lower bound on $f$-divergence,
$f$-GAN \cite{nowozin2016f} generalizes the generative adversarial networks (GAN) \cite{goodfellow2014generative} by using any  divergence measure from the  $f$-divergence family instead of cross-entropy as the discriminator.} 
$f$-GAN is an iterative optimization scheme for matching an implicit distribution $Q$ to a fixed distribution $P$ using any $f$-divergence. For a fixed $f$-divergence, the corresponding minmax optimization is, 
 \begin{equation}\label{eq:fGAN}
     \min_{Q} \max_{T_\omega} \mathbb{E}_{x\sim P}[T_\omega(x)] - \mathbb{E}_{x\sim Q}[f^*(T_\omega(x))]
 \end{equation}{}
 where $T_\omega:\mathcal{X}\mapsto\mathbb{R}$.


Recent approaches in IL applies  eq.~\ref{eq:il} to estimate  $\psi^*(\rho^{\pi} - \rho^{\pi_E})$ using various divergence measures, e.g.,  JS-divergence for GAIL \cite{GAIL} and reverse-KL in \cite{ke2019imitation}. In this work, we aim at \textbf{generalizing the definition of $\psi^*$} and \textbf{searching for the optimal $f^*$'s that fits various tasks}.

==> related.tex <==

\textbf{Inverse Reinforcement Learning.} Viewing the IRL problem as some kind of divergence minimization is not uncommon and yields multiple successful applications \cite{abbeel2004apprenticeship,dziugaite2015training,li2015generative,fu2017learning,GAIL,ke2019imitation,ghasemipour2019divergence}. 
Early works in IRL focuses on matching feature expectations \cite{abbeel2004apprenticeship} between expert and learner policies where the cost is a linear combination of the features. 
Maximum Entropy (Max-Ent) IRL \cite{ziebart2008maximum,ziebart2010modeling} is an energy-based model addressing degeneracies of the original IRL formulation \cite{ng2000algorithms,russell1998learning}. It naturally solves the IRL problem with moment matching and has multiple applications \cite{finn2016guided,wulfmeier2015maximum}. Though successful in low dimensional tasks, these methods does not scale well \cite{GAIL}.

For better scalability, \cite{fu2017learning,GAIL,finn2016connection} combines the Max-Ent IRL approach with the adversarial training idea \cite{goodfellow2014generative}, and demonstrates the IL problem an occupancy measure matching problem with JS divergence. \cite{ke2019imitation,ghasemipour2019divergence} further extended these works motivated by recent insights from generative modeling \cite{nowozin2016f}. They present a unified perspective of viewing the IL problem as occupancy measure $f$-divergence \cite{lin1991divergence,liese2006divergences,csiszar2004information} minimization problem. However, these works only try out several divergences on their performances as objectives quantifying the differences between expert and learner behaviors instead of giving a detailed analysis on which divergence works better in a certain task. 

In contrast, we %view IL as $f$-divergence minimization between learner and expert and 
strive to find an optimal $f$-divergence that always capture the maximum discrepancy perspective of expert and learner behaviors. 
Our approach is applicable to IRL approaches with different principles such as relative entropy \cite{boularias2011relative} or symmetric cross-entropy \cite{rhinehart2018r2p2}. 


%\textbf{Functional Optimization.} 
% Optimization over a function space is a case in functional optimization \cite{sasane2016optimization}. Solving it requires the expression of the admissible solution space of viable similarity measures (see more details in \cite{ritz1909neue}). Traditional ways to express the solution space adopts the fixed-structure parameterized (FSP) functions including a linear subspace (i.e., linear combination) of fixed basis functions \cite{ritz1909neue} or parameterized basis functions  \cite{zoppoli2002approximating,juditsky1995nonlinear} in the admissible solution space, and multi-hidden layer networks \cite{zoppoli2019neural}. %
%However, none of these works, to the best of our knowledge solves the problem of finding optimal $f$-divergence for IL problem. In our work, we are the first to learn an optimal $f$-divergence as an IL similarity measure using the FSP solution. We apply the input convex neural network \cite{amos2017input} and combine with a final short cut to express the $f$-divergence space for the optimization of maximum divergence discovery.
